GSN: Generalisable Segmentation in Neural Radiance Field

Traditional Radiance Field (RF) representations capture details of a specific scene and must be trained afresh on each scene. Semantic feature fields have been added to RFs to facilitate several segmentation tasks. Generalised RF representations learn the principles of view interpolation. A generalised RF can render new views of an unknown and untrained scene, given a few views. We present a way to distil feature fields into the generalised GNT representation. Our GSN representation generates new views of unseen scenes on the fly along with consistent, per-pixel semantic features. This enables multi-view segmentation of arbitrary new scenes. We show different semantic features being distilled into generalised RFs. Our multi-view segmentation results are on par with methods that use traditional RFs. GSN closes the gap between standard and generalisable RF methods significantly. Project Page: https://vinayak-vg.github.io/GSN/

==> src/figures/supp_moreclip.tex <==
\begin{figure*}[!ht]
    \begin{minipage}{0.24\linewidth}
        \centering
        \begin{tikzpicture}
            \node[anchor=south west,inner sep=0] (image) at (0,0) {\includegraphics[width=\textwidth]{assets/images/supplementary/moreclip/cake000.png}};
        \end{tikzpicture}
    \end{minipage}
    \begin{minipage}{0.24\linewidth}
        \centering
        \begin{tikzpicture}
            \node[anchor=south west,inner sep=0] (image) at (0,0) {\includegraphics[width=\textwidth]{assets/images/supplementary/moreclip/a piece of cake.png}};
        \end{tikzpicture}
    \end{minipage}
    \begin{minipage}{0.24\linewidth}
        \centering
        \begin{tikzpicture}
            \node[anchor=south west,inner sep=0] (image) at (0,0) {\includegraphics[width=\textwidth]{assets/images/supplementary/moreclip/steel_spoon.png}};
        \end{tikzpicture}
    \end{minipage}
    \begin{minipage}{0.24\linewidth}
        \centering
        \begin{tikzpicture}
            \node[anchor=south west,inner sep=0] (image) at (0,0) {\includegraphics[width=\textwidth]{assets/images/supplementary/moreclip/plate.png}};
        \end{tikzpicture}
    \end{minipage}
    
    \caption{\label{fig:supp_moreclip} In this figure, we show more results on a scene containing many objects. The first image shows the ground truth image of the scene. The next three images show the heat-map that we get when we give the text prompts {\em a piece of cake}, {\em a spoon}, and {\em a plate} respectively.}

\end{figure*}


==> src/sections/1_old_introduction.tex <==
\section{Introduction}
{

Capturing, digitizing, and authoring elaborate structures of real-world scene settings is a tedious task. The digitized scenes of the real world open a plethora of applications specifically in the field of graphics and augmented reality. To capture real-world scenes, initial efforts were made towards capturing the geometric content and its associated appearance via specialized hardware[CITE LIDAR and Appearance capturing modules]. Later efforts built on the ideas of epipolar geometry, structure from motion(SFM), and photometric stereo paved way for image-based capturing of the scenes. [CITE phototourism, phtometric stero SFM]. With the advent of Neural architectures, a relatively recent work of NeRF\cite{nerf} has shown photo-realistic novel views from a given set of discrete images. Follow-up works like [cite editing nerf, fast nerfs, compact nerf] have explored enhancing performance, editability, and memory requirements on the original work of \cite{nerf}. 

In most follow-up works of NeRF the representation of a scene is through a multi-layer perceptron (MLP) which is trained per scene. Later efforts like [CITE tensorf, plenoxels] have adopted a grid-based gradient optimization to represent the scene providing a faster optimization time. While these attempts are aimed towards faster and more accurate scene representation, they all lack generalization to various scenes, i.e; for every scene, the learning/optimization has to be re-done.

To address the aspects of generalization, few attempts were made namely [CITE Generatilzable nerf papers]. {\color{red} Write a line about each generalizatin work VINAYAK}.

While the works like GNT, NeRF, Plenoxels, and TensoRF provide ways to digitize the scene from a set of RGB images, often the interest of scenes is restricted to sub-parts of the captured scene. Whereby, one would require the 3D segmentation-based model to obtain the desired sub-parts. Initial works like [CITE some nerf segmentation papers], were made but a more recent approach ISRF[cite] presents a method by distilling semantic fields alongside radiance Fields, which allows interactive segmentation capabilities. Using this 3D segmentation, one can extract and utilize multi-view segmentation for various applications of artificial scene authoring. Similar to the approach of ISRF we also distill semantics into generalized Radiance Fields architecture. While ISRF is limited to scene-specific segmentation, we present a method  approach that allows the segmentation in a more generalized setting, which is not restricted to a particular scene. Moreover we incorporate various semantic encoding from various SOTA models and show results on our architecture.
[Last few lines needs refinement.]


Our approach provides generalized multi-view segmentations. Whereby,

\begin{itemize}
    \item We do not train the Radiance field and semantic field for every scene.
    \item We can perform multiview segmentation of Radiance feilds which is not specific to a scene.
    \item Finally, we show results of our framework on various semantic features and compare against the baseline scene specific segmentations models like ISRF.
\end{itemize}




}
